Locally Differentially Private Sparse Vector Aggregation

Vector mean estimation is a central primitive in federated analytics. In vector mean estimation, each user $i \in [n]$ holds a real-valued vector $v_i\in [-1, 1]^d$, and a server wants to estimate the mean of all $n$ vectors. Not only so, we would like to protect each individual user's privacy. In this paper, we consider the $k$-sparse version of the vector mean estimation problem, that is, suppose that each user's vector has at most $k$ non-zero coordinates in its $d$-dimensional vector, and moreover, $k \ll d$. In practice, since the universe size $d$ can be very large (e.g., the space of all possible URLs), we would like the per-user communication to be succinct, i.e., independent of or (poly-)logarithmic in the universe size. In this paper, we are the first to show matching upper- and lower-bounds for the $k$-sparse vector mean estimation problem under local differential privacy. Specifically, we construct new mechanisms that achieve asymptotically optimal error as well as succinct communication, either under user-level-LDP or event-level-LDP. We implement our algorithms and evaluate them on synthetic as well as real-world datasets. Our experiments show that we can often achieve one or two orders of magnitude reduction in error in comparison with prior works under typical choices of parameters, while incurring insignificant communication cost.

==> Makefile <==
# Switched this back to bibtex because the current version of crosstex
# seems to have a bug causing incorrect capitalization in the titles.

LATEX=pdflatex
TEXFLAGS=

TARGET=sparse-fl.pdf 
#TARGET2=leader-election-llncs.pdf 

#all: $(TARGET) $(TARGET2)
all: $(TARGET)
 

$(TARGET): $(TARGET:.pdf=.tex) tex/*.tex bibs/*.bib Makefile
	$(LATEX) $(TEXFLAGS) $<
	$(LATEX) $(TEXFLAGS) $<
#	bibtex $(basename $<)
#	bibtex $(basename $<)
#	$(LATEX) $(TEXFLAGS) $<
#	$(LATEX) $(TEXFLAGS) $<


full: $(TARGET:.pdf=.tex) tex/*.tex bibs/*.bib Makefile
	$(LATEX) $(TEXFLAGS) $<
	$(LATEX) $(TEXFLAGS) $<
	bibtex $(basename $<)
	bibtex $(basename $<)
	$(LATEX) $(TEXFLAGS) $<
	$(LATEX) $(TEXFLAGS) $<


$(TARGET2): $(TARGET2:.pdf=.tex) *.tex *.bib Makefile
	$(LATEX) $(TEXFLAGS) $<
	$(LATEX) $(TEXFLAGS) $<
	bibtex $(basename $<)
	bibtex $(basename $<)
	$(LATEX) $(TEXFLAGS) $<
	$(LATEX) $(TEXFLAGS) $<



test: test-fonts test-info

test-fonts: $(TARGET)
	pdffonts $<

test-info: $(TARGET)
	pdfinfo $<

print: $(TARGET)
	pdftops $< - | lpr -P lws510

view: $(TARGET)
	kpdf $<

clean:
	rm -f $(TARGET) *.out *.log *.aux *.bbl *.blg *.bak .*.xtx.cache parsetab.py \#*\# *~


==> tex/freq_est.tex <==
\section{Warmup: Sparse Binary Vector Mean Estimation}

\label{sec:binary-vector}
% \mz{This part only works for the item-level DP multi-item frequency estimation. Its utility can be fully covered by the continuous case. \textbf{It's relatively stable now.}}

%There are existing works on private single item frequency estimation that has logarithm communication cost, such as hash encoding scheme, and transformation scheme JL, Hadamard. 

We start from the discrete case where each user's vector contains only binary elements (i.e., $v\in \{0,1\}^d$, and $k\ll d$ elements are $1$).  We will present our method for the continuous setting in the next section.
% building the item-level LDP algorithm for a special case that all the input vectors are limited to $k$-sparse 01 vector. 
% In the following, we use the term ``item'' and ``coordinate'' interchangeably. %Some previous works \cite{wang2020set, privset} provide algorithms for the user-level LDP setting. 

%\noindent \textbf{Definition}. Each user $i$ holds a set $v_i$ consisting of $k$ items from domain $[d]$. The server wants to estimate the ``frequency'' of items -- for each item $x\in[d]$, $\bar{f}_x=\frac{1}{n}\sum_{i\in[n]}\mathcal{I}[x\in v_i]$. The $L_\infty$ error for estimation $\hat{f}$ is defined as $\max_{x\in[d]} |\hat{f}_x - \bar{f}_x|$. 

\noindent\textbf{Strawman Method (Repetition).}
To handle the case where each user has $k$ non-zero elements, the direct idea is to treat them as $k$ items. Each client repeatedly runs the one-item randomizer $\Q$ for those $k$ one-sparse vector and generates $k$ reports. The server simply uses the one-item aggregation algorithm $\mathcal{A}$ taking $k\cdot n$ reports (Alg~\ref{alg:blh} gives $\Q$ and $\mathcal{A}$) and multiply the result by $k$ (because $\mathcal{A}$ divides the sum by the total number of reports, $k\cdot n$, but we only have $n$ users). As a result, the $L_\infty$ error contains a $\sqrt{k}$ blowup, and from Theorem~\ref{theorem:blh_error}, this method has an error of $O\left(\sqrt{\frac{k \log d}{\eps^2 n}}\right)$.

\noindent\textbf{Our Solution.}
The reason why the strawman scheme incurs an extra $\sqrt{k}$ error blowup is each user reports $k$ times.  Although the original $k$ values are different, after the local randomizer, they all can ``contribute'' to any item in the domain, and thus add $k$ pieces of LDP noise to each element of the domain.  
Our idea is to use a separation scheme, such that each report contributes to a subset of the domain (and thus the noise is reduced), thus reducing noise.  To this end, we propose a hash-based splitting scheme:
% For those $k$ noisy reports generated by a client, they represent different coordinates. Those reports can be dealt separately in aggregation. Then, a hash-based splitting scheme comes in. 
Each user $i$ randomly samples a hash function $h^i: [d] \to [k]$ to divide the domain into $k$ disjoint subsets (we call them ``buckets'').\tw{we should say it's not necessarily $k$ buckets here. shall we use $b$?}  Ideally, $k$ non-zero items are distributed to $k$ buckets (we will discuss the common case later).  Each user then use the local randomizer to report the value in each bucket.  By doing this each user's report only contribute $1$ piece of noise to the full domain (instead of $k$ times in the strawman method), thus reducing the error.


% How to deal with hashing collisions and empty buckets? It turns out that a very simple strategy can be used -- i
If a bucket is empty or contains more than one reports, a dummy report is placed (we can extend the domain to $[d+1]$ and $d+1$ is the dummy item). In expectation, the dummy item has zero impact on other items' estimation results. In this case, we call this bucket has been ``zeroed out''. 



Alg~\ref{alg:freq_local} gives the pseudo code for the reporting procedure.  It runs the one-item randomizer $k$ times and places coordinate $x$'s report in the $h^i(x)$-th bucket -- $B^i_{h(x)}\get \Q(x, \eps)$. It sends all buckets $B^i=(B^i_1,\dots, B^i_k)$ and the hash function $h^i$ to the server. 

Alg~\ref{alg:freq} shows the server-side aggregation procedure.  It scans through all different coordinate $x \in [d]$. For each $x$, client $i$'s buckets, the report will be placed in the $B^i_{h^i(x)}$. The server runs the one-item aggregation algorithm $\cA(B^1_{h^1(x)},\dots,B^n_{h^n(x)})$. The server then sets the estimation for coordinate $x$ as the output of the one-item aggregation algorithm.
The aggregation algorithm also needs to compute the probability that an item ``survives'' the zero-out process due to hash collision. If we model the hash function as a random oracle, the survival probability is $p=(1-\frac{1}{k})^{k-1}$. The aggregation algorithm can now scale the estimation by $1/p$ to remove the bias introduced by zero-out process.

%The traditional way to design private multi-item frequency estimation algorithm is sampling. That is, each client will sample one item from its item set or from the item universe, then use an efficient one-item randomizer to generate a report. The privacy of the sampled item are protected by the one-item randomizer. The privacy of the remaining items are trivially preserved. The server aggregates those reports and computes an estimation of the frequency. Assuming every client holds exactly the same number of items, $k$, these sampling algorithms output an unbiased estimation. However, due to the nature of sampling, the error of these algorithms is enlarged by at least a factor of $k$ or even $d$.

%We propose a simple yet effective transformation idea to design For the local randomizer part, see Alg~\ref{alg:freq_local}. 
% \gf{Also explain this in words and with a figure (We should have a running example).}

\begin{algorithm}
	\caption{Multi-item Randomizer based on One-item Randomizer $\Q$}\label{alg:freq_local}
	\KwIn{One user's input item set $v=\{x_1,\cdots, x_{k}\}$.} %The public parameter $\theta$. The one-item randomizer $r(\cdot)$.
	\KwOut{$B_1,\dots,B_k$: $k$ buckets of randomized reports. $h$: hash function.}
	%\If{$|V|<k$}{
	%	Randomly select a set $V^*$ of $k-|V|$ items from $[d+1,d+k]$ 
	%	$V \get V \cup V^*$ 
	%} 
	%Randomly pick $b$ items from $V$ without replacement and call this set $V_b$. 
	Init $B_1,\dots,B_k$\\
    Sample a $k$-wise independent hash function $h:[d]\to [k]$ \\
	\For{$i \in [k]$}{
		$S_i = \{x|x\in v, h(x)=i\}$ \\
		\uIf{$S_i$ has exactly one item $x$}{
			%\tcp{Invoke one-item randomization algorithm to generate item $v$'s report}
			$B_i \get 
			\Q(v, \eps; \theta)$ 
		}
		\Else{
			%Generate a dummy report $r$ 
			%\tcp{Generate a dummy report}
			%Let $\perp$ be $d+1$ 
			$B_i \get 
			\Q(d+1, \eps; \theta)$  
		}
	}
	Report $(h, B_1, \dots, B_k)$
\end{algorithm}

\begin{algorithm}
	\caption{Multi-item Frequency Estimation Algorithm based on Aggregator $\cA$}\label{alg:freq}
	\KwIn{User's input $\v=\{v_i: i\in [n]\}$, the privacy parameter $\eps$} %, and the confidence parameter $\beta > 0$.
	\KwOut{A frequency estimation vector $\hat{f} \in [0,1]^d$}
	%\textbf{Generation of public parameters: $\theta$} \\
	\textbf{Local randomization algorithm: }\\
	User $i$ invokes the multi-item local randomizer (Alg~\ref{alg:freq_local}) to generate its report $(h^i, B^i_1, \dots, B_k^i)$ \\
	\textbf{Aggregation algorithm: } \\
	%$p\get \frac{b}{k}(1-1/b)^{b-1}$ 
	$p \get (1-\frac{1}{k})^{k-1}$ \\
	\For{$x \in [d]$}{
		%$Z \get \emptyset$  
		%\For{$i \in [n]$}{
		%	Add report $T^i[h^i(v)]$ to $Z$ 
		%}
		%\tcp{Collect the possible reports from every client's table.} 
		%$Z\get $ 
		%\tcp{Invoke the aggregation algorithm for one-item estimation to generate the estimation for $v$.} 
		$f^*_x \get \cA(B^1_{h^1(x)}, B^2_{h^2(x)}, \dots, B^n_{h^n(x)})$ \\
		$\hat{f}_x \get \frac{1}{p}f^*_x$ 
	}
\end{algorithm}

\noindent\textbf{Privacy and Utility Analysis.}
% We informally describe the privacy of the randomizer Alg~\ref{alg:freq_local} and the utility of the aggregator Alg~\ref{alg:freq}. 
Given any neighboring input $v$ and $v'$ that differ in one\tw{two? it is one according to the def, but in discrete setting, this means one of the two vectors has $k-1$ non-zero elements; does that impact utility?} coordinate $x$, for any hash function, at most one bucket will have a different output distribution. 
The randomizer Alg~\ref{alg:freq_local} invokes the one-item randomizer with privacy budget $\eps$. 
% By sequential composition (Theorem~\ref{thm:seq_comp}), 
The whole randomizer thus is $(\eps,0)$-item-level-LDP. 

For client $i$, if $v_{i,x}=1$, the report of $x$ will be placed in bucket $B_{h(x)}$ with prob. $(1-1/k)^{k-1}$. As long as the one-item aggregator algorithm can estimate the count for the survived item, by scaling, it can estimate the unbiased true count of item $x$. Also, the survival probability is $O(1)$, so the error introduced by zero-out-then-scale process can be bounded by $O\left(\sqrt{\frac{\log d}{n}}\right)$ by the Chernoff bound. 

\begin{theorem}
	\label{theorem:local_multi_privacy}
	Let one-item randomizer $\Q(\cdot,\eps)$ be an $\eps$-DP randomizer w.r.t. the neighboring relation that for any pair $x, x'\in[d]$, it always holds $v\sim v'$. Then the randomizer (Alg~\ref{alg:freq_local}) is an $\eps$-item-level LDP randomizer. %w.r.t. the neighboring relation $\sim$ defined as the following: for any two item sets $v\sim v'$, $v$ and $v'$ differ in one item.% between $x$ and $V'$ is at most one. Here, edit distance is defined by the smallest operation number to change one set to the other, where one operation can be replacing one item with a different item, adding one item or deleting one item. 
\end{theorem}

%Now we introduce our full mechanism in Alg~\ref{alg:freq} for the multi-item frequency estimation problem. 
%From lemma~\ref{lemma:bridge} and Theorem~\ref{theorem:local_multi_privacy}, we know the mechanism, Alg~\ref{alg:freq}, is $\eps$-DP w.r.t to the neighboring relation defined as the following: two inputs $\v \sim \v'$ iff $\v$ and $\v'$ only differ in one client's item set, say $V_i\ne V'_i$, and the edit distance between $V_i$ and $V'_i$ is at most one. Next, we provide the theorems for its utility.

\begin{theorem}
	%If the aggregation algorithm $\cA(\cdot)$ that takes the one-item randomized report as input and outputs an unbiased estimation, then algorithm \ref{alg:freq} outputs an unbiased estimation. Also,
	If the aggregation algorithm $\cA(\cdot)$ outputs an unbiased estimation with $L_\infty$ error within $\eta$ with probability at least $1-\beta/2d$, the multi-item frequency estimation Algorithm~\ref{alg:freq} outputs an unbiased estimation within $O\left(\eta+\sqrt{\frac{\log(d/\beta)}{n}}\right)$ $L_\infty$ error with probability at least $1-\beta$.
\end{theorem}

We refer the reader to the appendix for the full proof. Instantiate the multi-item frequency estimation algorithm with the local randomizer and the aggregator in the binary hashing one-item estimation Alg~\ref{alg:blh}. Set the confidence parameter $\beta$ to be $o(1/d^2)$, we have that, with prob. $1-1/d$, the algorithm outputs an unbiased estimation with $O\left(\sqrt{\frac{\log d}{\eps^2n}}\right)$ $L_\infty$ error. 
% \gf{We should talk about why this doesn't dependend on $k$. My understanding is that it's because we re	port $k$ bins for each user, so we reduce that error by increasing communication. Is that right? This raises the natural question--if you randomly subsampled the reporting table to only include $\ell$ out of $k$ bins (thus reducing your communication cost), how would your error scale?}

% \gf{I think the separation into theorems 3.1 and 3.2 is really indirect and not very intuitive. We should have one theorem that states the guarantee for a noise mechanism + an aggregation algorithm. If needed, we can separate the proof into lemmas that include things like 3.1 and 3.2, but they are roundabout and currently hiding the point. }









==> tex/intro.tex <==
\section{Introduction}
\label{sec:intro}


% Typically, the view of an adversary depends on some sensitive input data.

Federated analytics attracts more attention nowadays. Building upon the differential privacy theory, which quantifies the output distribution similarity of the sensitive input processing function, the federated analytics framework provides rigorous privacy guarantee for individual users while conducting large scale data statistics analysis. Numerous analytics problems have been discussed under this setting, such as such as item frequency estimation \cite{}, frequent item mining \cite{}, key-value data aggregation \cite{} and so on. The private federated analytics framework has already been deployed in industry environment, such Google Chrome xxxx, Apple xxx and xxx. Moreover, private federated machine learning, such as supervised neural network training\cite{}, clustering\cite{}, reinforcement learning,\cite{}, can be built upon the federated analytics framework. Vector aggregation, as a fundamental task in federated analytics, can be generalized to a large amount of applications. For example, the item frequency estimation can be seen as a vector mean estimation problem, where each client represents the items using one-hot encoding. For the key-value statistics, each client can map different keys to the corresponding coordinates and compile the key-value sets into a numerical vector naturally. FedAvg, as one of the most-used training algorithm for federated learning, involves a important step that the server computes the average of the users' gradient vectors to perform a global model update. 


%similarity. Recently, local differential privacy (LDP) has drawn a lot of attention because it provides a strong threat model in which users do not directly share data with the server. There have been numerous topic discussed in the LDP setting, 
%One popular scenario of using LDP is in the federated learning setting~\cite{}\tw{may down tune a bit, since we don't have experiments for fl}, where users send gradients to a central server with LDP noise, and the central server aggregates the received data to perform model update.  
% In this case, the challenge is (1) the communication cost is large for each user because each user needs to send the gradients for each parameter of the model, and (2) the accuracy is poor because 
%In this paper, we study the fundamental problem of using LDP in federated learning, which is estimating the mean of vectors submitted by users.  Moreover, we assume each user's vector is sparse, meaning that only a small fraction of elements are non-zero in the vector.




%\noindent \textbf{Multi-item Frequency Estimation}. There are $d$ different items indexed from $1$ to $d$. Each client $i$ holds an item set $V_i$ whose size is at most $k$. The server wishes to compute the frequency $f(v)$ for each item $v$, i.e., $f(v)=\frac{1}{n}|\{i\in[n] \mid v\in V_i\}|$. The $L_\infty$ of an estimation $\hat{f}$ is defined by $\max_{v\in[d]} |f(v)-\hat{f}(v)|$. 
\iffalse
\begin{theorem}[DP Mechanism for Multi-item Frequency Estimation]
Define a neighboring relation~$\sim$ on a client's input space
such that $V_i \sim V_i'$ \emph{iff} their symmetric difference has size at most 1.
We give an $(\eps,0)$-differentially private mechanism such that
with probability $1-\beta$, the 
$L_\infty$ error is at most $O(\sqrt{\frac{\log(d/\beta)}{\eps^2 n}})$.
Moreover, the per-client communication cost is $O(k\log n)$.
\end{theorem}
\fi


%Our mechanism gives $L_\infty$ error of $\sqrt{\frac{\log(d/\beta)}{\eps^2n}}$with probability $1-\beta$ while being $(\eps,0)$-differentially private. Here, the neighboring relation is defined as the following: two inputs $\v\sim \v'$ iff $\v$ and $\v'$ only differ in one client $i$'s input -- $V_i$ and $V'_i$, and the edit distance between $V_i$ and $V'_i$ is at most one. The per-client communication cost is $O(k\log n)$. 

\noindent \textbf{Sparse Vector Mean Estimation}. Each user $i$ holds a real value vector $v_i \in [-1,+1]^d$ that has at most $k$ non-zero coordinates. The server wants to estimate the mean of those vectors.  The ground truth is  $\frac{1}{n}\sum_{i\in[n]}v_i$, but due to the LDP noise, it is impossible to get the true result.  Instead, the server want an estimate as close to the ground truth as possible.  We use $L_\infty$ error to quantify the accuracy of the estiamte, which is defined as $\max_{j\in[d]} |\frac{1}{n}\sum_{i\in[n]}v_{i,j}-\hat{v}_j|$. 
% The sparse vector problem can be viewed as an extension of the frequency estimation problem. 


%
%Our mechanism gives $L_\infty$ error of $\sqrt{\frac{\log(nk/\delta)\log(d/\beta)}{\eps^2n}}$ with probability $1-\beta$ while being $(\eps,\delta)$-differentially private. Here, the neighboring relation is defined as the following: two inputs $\v\sim \v'$ iff $\v$ and $\v'$ only differ in one client $i$'s input -- $V_i$ and $V'_i$, and $\Vert V_i-V'_i \Vert_1 \le 1$. 
%


\noindent \textbf{Privacy Definitions}.
The widely accepted definition of LDP is known as \textit{user-level LDP}, in which the output distribution of the encoding algorithm (also referred to randomizer) is similar for any pair of possible inputs a user can possess. However, user-level LDP has poor utility guarantees for high-dimensional data analytics~\cite{}. A more relaxed definition is called \textit{event-level} LDP setting, in which the output distribution of the randomizer only needs to be similar for any pair of inputs that differ in one item (one element of the vector). None of the event-level LDP nor user-level LDP are designed for vector-type input. For numerical vector input, a more natrual way to define neighboring relation is through the distance between two vectors, such as $L_1$ or $L_2$ distance. In this paper, we define $L$-LDP --  two vectors are defined as neighboring if their $L_1$ distance is at most $L$. The $L$-LDP is more general and it can capture the essence of both of the event-level LDP and user-level LDP. 
% for all ``neighboring input pairs''. The neighboring input pairs are defined similarly as the central DP model -- two high-dimensional inputs are viewed as neighboring if they only differ in one item/coordinate/dimension. 
% The event-level LDP model can be seen as a tradeoff between privacy and utility -- it relaxes the privacy guarantee and generally has better utility guarantees. 
In this paper, we consider propose a unified framework that can be easily configured to be $L$-LDP. 

% Many data analytic problems' input can be modeled as vector, such as .... which makes vector aggregation a very important problem. Sparsity appears in practical use cases naturally, such as ....In this paper, we focus on designing LDP algorithms for estimating the mean of sparse vectors.

%A randomizer takes sensitive data as input and output a randomized report. 


%\gf{We should separate the problem statements from the results, and state the results in context of known lower bounds. A table would be nice.}








%%%%% The following definitions are now discared.
\iffalse
\mz{The following definitions are more conventional.}

\begin{definition}[Differential Privacy]
	An algorithm $\algA$ is an $(\eps,\delta)$-differntial private algorithm iff for any pairs of input $v, v'$ in the domain of $\algA$, where $v$ and $v'$ are neighbors, and for any $S\subseteq Range(A)$, it holds
	$$\Pr[\algA(v) \in S] \le e^\eps \Pr[\algA(v')\in S]+\delta$$
\end{definition}

For different problem settings, the meaning of ``neighbor'' can be varied. 

The local model is a specified computation model for client-server computation. Here, we will focus on the non-interactive version of local model. We also allow some form of public randomness. 

\begin{definition}[Local Model]
	An algorithm $\algA$ in local model accesses to a sensitive input set, $(v_1,\cdots,v_n)$ via the invocations of a local randomizer $\algR$. That means,  $$\algA(v_1,\dots,v_n)=\algA(\algR_\theta(v_1;\theta,r_{pub}),\dots,\algR_\theta(v_n;r_{pub})).$$ Here,
	$\theta$ represents the public parameters and $r_{pub}$ is the public random tape represented by an infinite 01-tape.
\end{definition}

\begin{definition}[Local Diffrential Privacy]
	An algorithm $\algA$ in local model is $(\eps,\delta)$-local differential private algorithm iff for any revelation of the public random tape $r_{pub}$, the local randomizer $\algR(\cdot;r_{pub})$ is $(\eps,\delta)$-differential private.
\end{definition}

\mz{The following definitions are more inclusive and general.}
\fi


\subsection{Existing Approaches}

% We specifically focus on the non-interactive local differential private sparse vector mean estimation problem. There are many existing works on closely related settings and among those algorithms, some can be easily extended or modified to fit the definition of our problem. 

To solve the estimation problem in the event-level LDP setting,  one can directly extend the single-item LDP algorithms, such as hash encoding~\cite{wang2017locally}, Hadmard Response~\cite{cormode2018marginal}, and Johnson-Lindenstrauss Transformation method~\cite{bassily2015local}. These algorithms achieve the same and optimal error in the single-item setting with logarithmic communication cost. Simply repeating these methods for each item, i.e., the client runs these algorithms for each non-zero coordinate and submit all reports to the server, solves the problem. 
For the user-level LDP setting, a simple sampling protocol is possible: the user randomly samples one non-zero coordinate, runs the one-item algorithm and submits the single report. 

For numerical vector mean estimation, one can use the widely-used Gaussian mechanism~\cite{GaussianMech}\tw{why don't we consider Laplace, since all other methods are pure LDP}. However, its communication cost is proportional to the dimension of the vector $d$. There are also methods based on user-level LDP, such as Harmony~\cite{harmony}, PM and HM~\cite{WangNing2019}. Asymptotically, they achieve the same and optimal error in non-sparse setting and have logarithmic communication cost. However, none of them exploit the sparsity property of the problem we consider. 

The most related line of work is LDP key-value mean value estimation. In that setting, each client has at most $k$ key-value pairs and the server wishes to compute the mean value for every single key. This setting is almost the same as our sparse vector mean estimation. 
The difference is, in the key-value setting, the server only estimates the mean value for those clients that holds the corresponding key (divide the sum by number of users that possess the key), while we compute the mean value for all the clients (divide the sum by the total number of users $n$).  
In other words, the two problems are equivalent if we consider sum, but are different in terms of mean, because the dividents are different.
Nonetheless, given a proper scaling process, as we describe later, those algorithms can be applied to sparse vector mean estimation. 
We focus on non-interactive setting, so we choose to compare with PCKV~\cite{pckv} and not to compare with PrivKV~\cite{privkv} and PrivKVM~\cite{privkvm}, which are multi-round interactive algorithms. 


\begin{table*}[ht]
\label{tab:comp1}
\centering 
\begin{tabular}{c|cc|cc}
\toprule
\multirow{2}{*}{\textbf{Name}} & \multicolumn{2}{c|}{\textbf{Event-level LDP}}   & \multicolumn{2}{c}{\textbf{User-level LDP}}   \\ 
  & \textbf{Comm. Cost} & \textbf{$L_\infty$ Error} & \textbf{Comm. Cost} & \textbf{$L_\infty$ Error} \\ \midrule
$k$-fold Repeating & $O(k\log d)$ & $O\left(\frac{1}{\eps}\sqrt{\frac{k\log d}{n}}\right)$ & - & - \\ 
Sampling & - & - & $O(\log d)$ & $O\left(\frac{k}{\eps}\sqrt{\frac{\log d}{n}}\right)$ \\ 
Gaussian\cite{GaussianMech} & $O(d)$ & $O\left(\frac{1}{\eps}\sqrt{\frac{\log(1/\delta)\log d}{n}}\right)$ & $O(d)$  & $O\left(\frac{k}{\eps}\sqrt{\frac{\log(1/\delta)\log d}{n}}\right)$ \\ 
Harmony\cite{harmony} & - & - & $O(\log d)$  & $O\left(\frac{1}{\eps}\sqrt{\frac{d\log d}{n}}\right)$ \\ 
PCKV\cite{pckv} & - & - & $O(\log d)$  & $O\left(\frac{1}{\eps}\sqrt{\frac{d\log d}{n}}\right)$ \\ 
Ours & $O(k \log k)$ & $O\left(\frac{1}{\eps}\sqrt{\frac{\log d}{n}}\right)$ & $O(\log k)$  & $O\left(\frac{1}{\eps}\sqrt{\frac{k\log n\log d}{n}}\right)$ \\ \midrule
Lower Bounds & - & $\Omega\left(\frac{1}{\eps}\sqrt{\frac{\log d}{n}}\right)$ & - & $\Omega\left(\frac{1}{\eps}\sqrt{\frac{k\log d}{n}}\right)$ \\ \bottomrule
\end{tabular}
\caption{Comparison with Existing Approaches} % title of Table
\end{table*}

\subsection{Our Results}

To handle sparse vector estimation, we first propose a general LDP definition that bridges the gap between event-level and user-level settings. Our definition uses $L_1$ distance as the metric to define neighboring vector. 
We then provide a unified and configurable algorithm to tackle the sparse vector mean estimation problem under both event-level and user-level settings. Our algorithm combines multiple techniques, including hash-and-binning and random sign flipping to generate a short vector that can be seen as an encoding of the original vector. Then, our algorithm adds Laplacian noise to the short vector. 
By comparing with existing lower bound of estimation error, we show that our algorithm has optimal estimation error in event-level LDP setting. 
Finally, we provide a new lower bound of error for sparse vector mean estimation under user-level LDP setting. Our estimation algorithm has nearly-optimal utility guarantee that only has an extra $O(\sqrt{\log n})$ factors in the $L_\infty$ error. 
The asymptotic comparison for the existing work is shown in table~\ref{tab:comp1}.

% When two vectors' distance is not larger than $L$, we define them as neighboring. The event-level DP can be captured by a very small $L$ value. For example, if the input vector is bounded by $[-1,+1]$ in each coordinate, then two neighbor vectors that only differ in one coordinate will have $L_1$ distance of at most 2. Therefore, by setting $L=2$, we have a slightly more general neighboring definition and 

%We start from building the event-level DP algorithm. The natrual idea, which is our strawman algorithms, simply decomposes the $k$-sparse vector into $k$ one-sparse vector. Then, we can view each client as the proxy of $k$ ``virtual clients''. The client simply repeatedly run the one-item randomizer for those $k$ one-sparse vector and generates $k$ reports. The server simply views the reports as they generated by $nk$ virtual clients, then runs the one-item aggregation algorithm to generate an estimation. Finally, the server scales the estimation mean vector by a factor of $k$, which then 

\iffalse
We can modify the LDP primitives for the single-item setting to the multi-item setting (here we only consider the multi-item frequency estimation problem):
\gf{This discussion of different types of LDP and results does not belong here (move later) and should be rewritten. In the introduction, we should have one subsection with our results, where we pick the most representative results from each problem.}
\begin{itemize}
    \item RAPPOR can be easily extended to event-level LDP, because two neighboring values differ in two locations, and the proof or RAPPOR can easily capture that.
    \item For user-level LDP, if two neighboring values differ in $2k$ locations, directly extending RAPPOR results in a privacy loss of $k\epsilon$.  It seems the best method is to first sample $1$ out of $k$ values, and then use the single-item RAPPOR, and scale the results by $k$.  But this gives a error blow-up of $k$.
    \item For user-level LDP, we can modify RR and Hashing to a ``combined-encoding'' version.  Specifically, in the original RR, there is only one high bar (with probability $\frac{e^\epsilon}{e^\epsilon + d - 1}$, the true answer will be transmitted.  Here we have $k$ high bars corresponding to the $k$ items, each with a height of $\frac{e^\epsilon}{ke^\epsilon + d - k}$.  Further proofs show that this method incurs a $\sqrt{k}$ error blow-up.
    \item It seems there is no one-to-one correspondence between RAPPOR and Hash in the multi-item setting.
    \item We propose a binning strategy for RR and Hashing.
\end{itemize}


\begin{table*}[!h]
\centering
\footnotesize
\begin{tabular}{c|c|c}
% \toprule
       & event-level             & User-Level\\
       \midrule
RR     & Binning (this paper): $1, k$ &    Combined Reporting: $\sqrt{k}, 1$    \\
RAPPOR & Direct Extension: $1, d$       & Sampling: $k, d$ \\
Hashing& Binning (this paper): $1, k$   & Combined Reporting~\cite{wang2020set}: $\sqrt{k}, \log d$
%\bottomrule
\end{tabular}
\normalsize
\caption{A summary of variants in different settings and their respective error blow-up factor and communication cost.
}
\label{tbl:summary}
\end{table*}
\fi

==> tex/related-elaine.tex <==
\subsection{Additional Related Work}

\elaine{TODO: write}


==> tex/related.tex <==
\section{Related Work}
\label{sec:related}
\paragraph{Categorical Data Collection.}
The building block of categorical data collection is frequency oracle, where each user possesses a categorical value, and the aggregator aims to estimate the frequency of all values within the domain. 
The first (and probably the most basic) mechanism is randomized response~\cite{randomizedresponse}.
The major shortcoming of randomized response is that when the domain size is large, the utility will be poor, because most of the users will randomize their values to another value.

To handle the large domains, one approach is called RAPPOR:  it encodes the value into a bit-vector where only one location is 1 (i.e., one-hot encoding).  
By doing this, the domain size of any location is only 2, and one can then use randomize response to each bit~\cite{rappor}. Variants over RAPPOR are also studied to improve its utility~\cite{wang2017locally,optimalschemes2018Ye}.
However, this approach suffers from the high communication cost because users need to send the whole bit-vector, which has size proportional to the domain size.

To handle the large communication cost, another approach is to ``compress'' the domain.  Bassily and Smith~\cite{bassily2015local} used the Johnson Lindenstrauss (JL) transformation as the compressing tool.  
Hadamard transformation is also used~\cite{Bassilynips2017,2018Hadamard}.  
Wang et al.~\cite{wang2017locally} presented a hashing function-based perspective of these methods and extended it from outputting $\pm 1$ in JL or Hadamard to outputting more values.
However, this approach reaches the optimality only when $e^\epsilon$ is an integer.  
More recently, researchers also propose methods that obtain optimality for any $\epsilon$ value~\cite{wang2020set,feldman2021lossless}.


\paragraph{Numerical Data Collection.}
Recent work on numerical data collection under LDP also investigates mean estimation when the users' private values are numerical/continuous.
In Duchi et al.~\cite{duchi2018minimax}, the authors propose to first randomly discritize the value into one of the two extreme points within the range, and then apply binary randomized response.
The rounding step loses too much information because it always gives 1 bit as the output.
Thus, when $\epsilon$ is large, this approach suffer from poor utility.
Wang et al.~\cite{WangNing2019} propose the piecewise mechanism where the output is continuous and randomly distributed within the domain; it achieves better utility than Duchi's method~\cite{duchi2018minimax} when $\epsilon>1.29$.  
A similar method is also proposed in Li et al.~\cite{li2020numeric}.
More recently, Zhao et al. bridged the gap between Duchi et al. and the piecewise mechanism~\cite{zhao2020local} by 
(1) extending the Duchi's method by allowing the stochastic rounding step to output three (instead of two) possible values, which outperforms the original method when $\epsilon>0.69$, and 
(2) deriving better parameters for the piecewise mechanism.

\paragraph{Handling Set-Values.}
When each user possesses more than one values, the standard approach is to ask users to sample one item to report (e.g., \cite{qin2016heavy,wang2018locally}) treating the underlying one-item reporting protocol (reviewed above) as a black-box.  But this introduces an error blowup factor of $k$.  Wang et al. proposed PrivSet\cite{wang2018privset} that generalizes exponential mechanism to set values, but their algorithm involves large combinatorial number computing, which is generally impractical for large $d$ case. 

In the event-level LDP setting, the straightforward approach is to ask each user to report $k$ times (thus each user is treated as $k$ users).  This introduces a $\sqrt{k}$ error blowup factor.  Another straightforward approach is to modify the RAPPOR-based method, so that each bit-vector has $k$ 1's.  By doing this, the error bound is the same as original method in the single-item setting, but the communication cost is high.

\paragraph{Other Definitions.} 
In~\cite{arxiv:erlingsson2020encode}, the authors proposed the notion of removal LDP.  
The ``removal'' intuition originates from the traditional, centralized DP, where we want to hide/protect whether a particular user contributes to the data publication or not.
In LDP, each user adds noise onto their own values and report it to the server, so the server naturally knows whether a user contributes or not.
Erlingsson et al. argued that sending a pre-defined null/dummy values can be seen as non-contribution.

Wang et al. propose to relax the definition by taking into account the distance between the true value and the perturbed value~\cite{wang2017local_ordinal} (similar to the geo-indistinguishability notion in the centralized setting~\cite{andres2012geo}).
More formally, given the true value, with high probability, it will be perturbed to a nearby value (with some pre-defined distance function); and with low probability, it will be changed to a value that is far apart.  
A similar definition is also proposed in other work~\cite{gursoy2019secure,gu2019supporting}. 

Another setting where some answers are sensitive while some not is also investigated~\cite{murakami2019utility} (there is also a DP counterpart called One-sided DP~\cite{doudalis2017one}).  
Later Gu et al. proposed a more general version~\cite{gu2019providing} that allows different values to have different privacy level.
Finally, Yue et al. proposed a version that combines metric~\cite{murakami2019utility} and private-public separation~\cite{wang2017local_ordinal} and use it to perturb texts~\cite{ACL21/YueDu21}.

\tw{tw add distributed dp}\cite{bonawitz2017practical,bagdasaryan2021towards}


==> tex/roadmap-mingxun.tex <==
\section{Technical Roadmap}
In this section, we give an informal technical overview of our results.

\subsection{Warmup: an Event-Level LDP Mechanism for Frequency Estimation}

For simplicity, we 
first focus on 
the special case of designing a {\it frequency estimation}
mechanism that satisfies {\it event-level} LDP.
Recall that the frequency estimation problem is a special
case of our general formulation of vector mean estimation. 
In frequency estimation, each client $i \in [n]$ has a binary vector 
$v_i \in \{0, 1\}^d$, 
denoting whether the client owns each item from a universe of $d$ items.
The server wants to estimate the frequency of each item.
Once we understand how to design an event-level LDP mechanism
for frequency estimation, we can later 
extend our techniques to 1) support {\it user-level} LDP; and 2)
support the more general case of vector mean estimation
where the client's vector is from a real domain.


\paragraph{Strawman: $k$-fold repetition of the $1$-sparse scheme.}
Recall that prior works~\cite{bassily2015local, wang2017locally, cormode2018marginal} have proposed $1$-sparse frequency estimation mechanisms
that achieve optimal error, that is, $\widetilde{O}(\frac{1}{\epsilon \sqrt{n}})$ 
error, incurring only $\widetilde{O}(1)$ communication.
In our problem, each client
owns $k$ items rather than $1$.
Therefore, a strawman idea 
is through a $k$-fold repetition of the $1$-sparse scheme~\cite{}.
Specifically, each client can pretend to be 
$k$ virtual clients, and each 
virtual client owns only one item. 
Imagine that we run a $1$-sparse scheme over these $k n$ virtual clients.  
Since each client acts as $k$ virtual clients, its communication cost
is $\widetilde{O}(k)$ which is independent of the universe size $d$.
The resulting error 
would be $\widetilde{O}(\frac{1}{\epsilon \sqrt{k n}})$ --- however,
keep in mind that here, the mean is taken over all $k n$ virtual clients.
In reality, we want to take the mean over the $n$  
real clients. Thus, after renormalizing, the 
actual error would be  
$\widetilde{O}(\frac{\sqrt{k}}{\epsilon \sqrt{n}})$.

This strawman scheme gives non-trivial bounds,  
but the error is not optimal. Recall that we are aiming to
achieve optimal 
$\widetilde{O}(\frac{1}{\epsilon \sqrt{n}})$ error. 



\paragraph{Our idea.}
We devise a new scheme which makes {\it non-blackbox} usage of 
the elegant ideas behind the $1$-sparse
mechanism by Wang et al.~\cite{wang2017locally}, 
combined with a new random binning idea.
Our idea is as follows:
\begin{itemize}[leftmargin=3mm]
\item
\underline{\it Each client} $i \in [n]$ 
does the following:
\begin{enumerate}[leftmargin=3mm]
\item Sample two random hash functions 
$h_i : [d] \rightarrow [k]$
and $s_i : [d] \rightarrow \{-1, 1\}$.
\item 
Let $\{x_1, \ldots, x_k\}\in [d]^k$
denote the $k$ items belonging to client $i \in [n]$. 
For each $j \in [k]$, place $x_j$ into the hash bin  
indexed $h_i(x_j)$. Note that in total, there are $k$ hash bins per client.
\item 
For each hash bin $j \in [k]$, compute
$B_{i, j} := \sum_{x \in \text{bin } j } s_i(x) + {\sf Lap}(\frac{1}{\epsilon})$
where ${\sf Lap}(\frac{1}{\epsilon})$
denotes Laplacian noise of average magnitude 
$\frac{1}{\epsilon}$.
\item 
Send to the server the tuple $(\{B_{i, j}\}_{j \in [k]}, h_i, s_i)$ where $h_i$ and $s_i$ denote
the description of the two hash functions.
\end{enumerate}
\item
\underline{\it Server} does the following to estimate the fraction 
of clients that own an arbitrary item $x^* \in [d]$:
\begin{enumerate}[leftmargin=3mm]
\item 
For each client $i \in [n]$, compute $j^* = h_i(x^*)$. 
\item 
Output $\frac{1}{n}\sum_{i \in [n]} B_{i, j^*} \cdot s_i(x^*)$.
\end{enumerate}
\end{itemize}

As mentioned later, to get our desired bounds, 
we need the hash functions 
$h_i$ and $s_i$ be pseudorandom --- however, we stress
that the pseudorandomness assumption is needed only 
for deriving stochastic bounds
and not needed for proving privacy.
In other words, our scheme satisfies information-theoretic LDP.
Specifically, 
to sample a pseudorandom function, the client
simply has to sample a random seed whose 
length is proportional to a security parameter and independent of $d$.
To send the description of the hash function to the server,
the client simply sends the pseudorandom seed 
to the server (since we only use pseudorandomness 
for measure concentration and not for privacy, 
it is safe for the client to just send the pseudorandom seeds
to the server).


\paragraph{Informal error analysis.}
To gain intuition, we present an informal analysis of our scheme.
The formal proofs (for the more generalized vector mean estimation scheme) 
are deferred to Section~\ref{sec:sparse-vec}. 
%and the proofs are presented
%for the more generalized version where each client's vector may be from
%a real domain. 
%\elaine{fwd ref}
Note that understanding the error analysis also helps to 
understand why the scheme works.

Henceforth, we 
use $(i, j)$ to denote the $j$-th bin of client $i$.
Let $C_{i, j} = \sum_{x \in \text{bin } (i, j)}s_i(x)$
be the true aggregated ``count''
of the $j$-th bin belonging to the $i$-th client.
Suppose that the server wants to know the 
frequency of item $x^* \in [d]$.
To do this, the server computes the summation 
%$\sum_{i \in [n]} R_{i, h_i(x^*)} \cdot s_i(x^*) = 
%\sum_{i \in [n]} \sum_{x \in \text{bin } 
%(i, h_i(x^*))} s_i(x)\cdot s_i(x^*) + \sum_{i \in [n]}{\sf Lap}(\frac{1}{\epsilon})$.
$\sum_{i \in [n]} B_{i, h_i(x^*)} \cdot s_i(x^*) = 
\sum_{i \in [n]} C_{i, h_i(x^*)}
\cdot s_i(x^*) + \sum_{i \in [n]}{\sf Lap}(\frac{1}{\epsilon})$.
The second part, $\sum_{i \in [n]}{\sf Lap}(\frac{1}{\epsilon})$ 
is a noise of magnitude roughly $\widetilde{O}(\frac{\sqrt{n}}{\epsilon})$, 
whereas the first part 
%$\sum_{i \in [n]} \sum_{x \in \text{bin } (i, h_i(x^*))} s_i(x)\cdot s_i(x^*)$
$\sum_{i \in [n]} C_{i, h_i(x^*)}
\cdot s_i(x^*)$
can be decomposed into two sources of contributions:
\begin{enumerate}
\item  
Each client $i$ who owns $x^*$
contributes one $+1$ term to the summation.
\item 
For each client $i$ and each item $x \neq x^*$ 
owned by the client 
such that $h_i(x) = h_i(x^*)$, 
it contributes a random choice of 
$-1$ or $+1$  
to the summation, assuming that $s_i(\cdot)$ is a random oracle.
\end{enumerate}
Thus, 1) corresponds to 
to the true count of the item $x^*$, 
whereas 2) is can be viewed as the result 
of a random walk of expected length $O(n)$, 
i.e., a random noise of magnitude roughly $\widetilde{O}(\sqrt{n})$.
In particular, the length of this random walk is upper bounded by the total
load of the hash bins $\{(i, h^*(i))\}_{i \in [n]}$, which is $O(n)$
assuming that each $h_i$ is a random oracle.

Summarizing the above, the estimated count  
is the true count plus roughly $\widetilde{O}(\frac{\sqrt{n}}{\epsilon})$ noise.
\elaine{note:this expression 
makes some assumption on the range of epsilon}
Finally, when the server normalizes
the above sum by $\frac{1}{n}$ to compute the average, the resulting error becomes 
$\widetilde{O}(\frac{1}{\epsilon \sqrt{n}})$.
At this point, it is helpful to observe that 
in this construction, the error comes from two sources --- this observation
will later help us to generalize the scheme to user-level LDP:
\begin{itemize}[leftmargin=5mm]
\item 
{\it Noise component:} the first source of error is the  
sum of $n$ independent ${\sf Lap}(\frac{1}{\epsilon})$ noises, 
one for each bin $(i, h_i(x^*))$
where $i \in [n]$;
\item 
{\it Contribution from irrelevant items:}
the second source of error is 
the random contribution of either $+1$ or $-1$ from each element 
$x \neq x^*$ that each client $i$ 
places into the bin $(i, h_i(x^*))$.
\end{itemize}


\begin{remark}
In the above, we assumed that the hash functions $h_i$'s and $s_i$'s
are random oracles. 
In practice, we can instantiate the hash functions using pseudorandom functions
where the pseudorandomness assumption is only needed for measure concentration
but not needed for privacy.
\end{remark}




\paragraph{Informal LDP analysis.}
We also give informal privacy analysis, while deferring
the formal proofs to Section~\ref{sec:sparse-vec}.
We want to show that the scheme satisfies $\epsilon$-event-level-LDP.
%First, we argue that the scheme satisfies $\epsilon$-event-level-LDP.
Fix the hash functions $h_1, \ldots, h_n, s_1, \ldots, s_n$, 
and consider two input configurations $\v, \v' \in \{0, 1\}^{d \cdot n}$
that differ in only one position. 
Let $C_{i, j} = \sum_{x \in \text{bin } j}s_i(x)$
be the true aggregated ``count''
of the $j$-th bin belonging to the $i$-th client, when the input configuration
is $\v$; and let $C'_{i, j}$ be the corresponding 
quantity when the input configuration is $\v'$.
It must be that all $C_{i, j}$
and $C'_{i, j}$ are 
the same everywhere except for one bin $j^*$ corresponding to one client $i^*$.
Moreover, for the only location where they differ, 
it must be that $|C_{i^*, j^*} - C'_{i^*, j^*}| \leq 1$.
Having observed this, it is not too hard to show 
that adding  Laplacian noise of average
 magnitude $\frac{1}{\epsilon}$ to each bin suffices
for achieving $\epsilon$-event-level-LDP.

\subsection{Extension: a User-Level LDP Mechanism for Frequency Estimation}
%We now generalize the above warmup scheme to support user-level LDP. 
One trivial way to obtain user-level LDP is to 
directly use the aforementioned warmup 
scheme, and simply apply the standard group privacy theorem~\cite{dworkrothdpbook} %\elaine{cite}
to reset the parameters.
Specifically, %for a total privacy budget of $\epsilon$, we will need to  
to achieve $\epsilon$-user-level-LDP, we would need to plug in  
a privacy  parameter of $\frac{\epsilon}{k}$ when invoking
the warmup scheme.
This results in an error bound of 
$\widetilde{O}(\frac{k}{\epsilon \sqrt{n}})$ which is an $\widetilde{O}(\sqrt{k})$
factor away from optimal.

\paragraph{Strawman: sampling + $1$-sparse mechanism.}
Another strawman idea for each client to randomly sample $1$ item out of its $k$ items,  
apply the $1$-sparse mechanism to the sampled items,   
and finally, renormalize the estimate accordingly. 
Unfortunately, it is not hard to show that the  
resulting error would be 
$\widetilde{O}(\frac{k}{\epsilon \sqrt{n}})$, also an $\widetilde{O}(\sqrt{k})$
factor away from optimal.

\paragraph{Our approach.}
Our approach is to  our warmup mechanism.
In the more general case, 
imagine that we want to achieve $(\epsilon, \delta)$-LDP 
under $L$-neighboring input configurations, and recall that user-level LDP
is simply a special case where $L = 2k$.
In other words, we want the server's view to be $(\epsilon, \delta)$-close
for two input configurations 
$\v = (v_1, \ldots, v_n) \in \{0, 1\}^{d\cdot n}$ and
 $v' \in (v'_1, \ldots, v'_n)  \in \{0, 1\}^{d\cdot n}$
under the distance notion 
of the standard $(\epsilon, \delta)$-differential privacy definition~\cite{}.
Two input configurations 
$\v = (v_1, \ldots, v_n) \in \{0, 1\}^{d\cdot n}$ and
 $v' \in (v'_1, \ldots, v'_n)  \in \{0, 1\}^{d\cdot n}$
are $L$-neighboring iff they differ in only one user's
contribution $v_i$ and $v'_i$, and moreover, 
$|v_i - v'_i|_1 \leq L$.
In our reasoning below, we will carry around the parameter $L$, 
and at the end, we can plug in $L = 2k$ to get the user-level LDP result.
However, as noted earlier in Section~\ref{sec:intro},
the more general scheme parametrized by $L$
can be of independent interest.

Our more generalized scheme is almost the same as the warmup scheme, except
with the following modifications:
\begin{itemize}
\item 
Each client now has $b$ hash bins
rather than $k$ bins as in the warmup scheme.
For the time being, we will leave the choice of $b$ unspecified,
and we can work out the optimal choice later.
\item 
Each client $i \in [n]$ now computes the noisy sum $R_{i, j}$ as 
$R_{i, j} := \sum_{x \in \text{bin } j } s_i(x) + {\sf Lap}(\frac{1}{\epsilon'})$
where $$\epsilon' = \frac{\epsilon}{\min(L, \sqrt{b L \log\frac{1}{\delta}})}$$
\end{itemize}

Consider two $L$-neighboring input configurations 
$\v$ and $\v'$, and fix all hash functions $h_1, \ldots, h_n$
and $s_1, \ldots, s_n$. When we change $\v$ to $\v'$,  
at most $L$ bins' true ``counts'' 
$C_{i, j} := \sum_{x \in \text{bin } (i, j) } s_i(x)$
are affected, and these $\min(b, L)$ bins must belong to the same client.
Furthermore, for each bin whose count is affected, 
the change in its true ``count''
is upper bounded by $\min\left(L, O(\sqrt{\frac{L\cdot \log\frac1\delta}{b}})\right)$
with probability $1-O(\delta)$.
\elaine{TODO: rewrite this explanation}



\subsection{Generalizing to Real-Valued Vectors}

\subsection{Our Lower Bound}



